A Fine-Grained Analysis on Distribution Shift

Robustness to distribution shifts is critical for deploying machine learning models in the real world. Despite this necessity, there has been little work in defining the underlying mechanisms that cause these shifts and evaluating the robustness of algorithms across multiple, different distribution shifts. To this end, we introduce a framework that enables fine-grained analysis of various distribution shifts. We provide a holistic analysis of current state-of-the-art methods by evaluating 19 distinct methods grouped into five categories across both synthetic and real-world datasets. Overall, we train more than 85K models. Our experimental framework can be easily extended to include new methods, shifts, and datasets. We find, unlike previous work~\citep{Gulrajani20}, that progress has been made over a standard ERM baseline; in particular, pretraining and augmentations (learned or heuristic) offer large gains in many cases. However, the best methods are not consistent over different datasets and shifts.

==> fixeddata.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/legend.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/dSprites;fixeddata.png}
    \caption{\dsprites (label = shape, attribute = color)}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/mpi3d;fixeddata.png}
    \caption{\mpithreed (label = shape, attribute = color)}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/shapes3d;fixeddata.png}
    \caption{\shapes (label = shape, attr = color)}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/smallnorb;fixeddata.png}
    \caption{\smallnorb (label = category, attr = azimuth)}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/camelyon;fixeddata.png}
    \caption{\camelyon (label = has tumor cells, attribute = hospital)}
    \end{subfigure}
    \caption{{\bf Condition 2: Fixed data size.} We plot the top-1 accuracy (y-axis) for different amounts of data. The total size of $\train$ is $T$. Higher is better. }
    \label{fig:fixeddata}
\end{figure}

==> noise.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/legend.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/dsprites;noise.png}
    \caption{\dsprites (label = shape, attribute = color)}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/mpi3d;noise.png}
    \caption{\mpithreed (label = shape, attribute = color)}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/shapes3d;noise.png}
    \caption{\shapes (label = shape, attr = color)}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/smallnorb;noise.png}
    \caption{\smallnorb (label = category, attr = azimuth)}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{graphs/camelyon;noise.png}
    \caption{\camelyon (label = has tumor cells, attribute = hospital)}
    \end{subfigure} 
    \caption{{\bf Condition 1: Noisy labels.}  We plot the top-1 accuracy (y-axis) for different amounts of noise. Labels are set to noise with probability $p$. Higher is better.}
    \label{fig:noisylabels}
\end{figure}
